Performance Bound Analysis for Crowdsourced Mobile Video Streaming

Adaptive bitrate (ABR) streaming enables video users to adapt the playing bitrate to the real-time network conditions to achieve the desirable quality of experience (QoE). In this work, we propose a novel crowdsourced streaming framework for multi-user ABR video streaming over wireless networks. This framework enables the nearby mobile video users to crowdsource their radio links and resources for cooperative video streaming. We focus on analyzing the social welfare performance bound of the proposed crowdsourced streaming system. Directly solving this bound is challenging due to the asynchronous operations of users. To this end, we introduce a virtual time-slotted system with the synchronized operations, and formulate the associated social welfare optimization problem as a linear programming. We show that the optimal social welfare performance of the virtual system provides effective upper-bound and lower-bound for the optimal performance (bound) of the original asynchronous system, hence characterizes the feasible performance region of the proposed crowdsourced streaming system. The performance bounds derived in this work can serve as a benchmark for the future online algorithm design and incentive mechanism design.

==> section-app.tex <==
%!TEX root = DASH_Main_JSAC.tex
%SourceDoc DASH_Main_JSAC.tex




\appendix

\section{Appendix}

\subsection{Proof for Proposition 1}
\subsection{Proof for Proposition 2}
\subsection{Proof for Proposition 3}
\subsection{Proof for Theorem 1}
\subsection{Proof for Theorem 2}








==> section2-literature.tex <==
%!TEX root = DASH_Main_CISS_new.tex
%SourceDoc DASH_Main_CISS_new.tex

\section{Literature Review}

%(1) Literature related to the mobile video services and DASH services ...
%\\
%
%(2) Literature related to the scheduling methods in the basic DASH model with a single user: (i) Buffer based, (ii) Channel prediction based, and (iii) End-to-end throughput prediction based.
%\\
%
%(3) Literature related to the advanced DASH models: (i) P2P model: Users buffer the played video data, which can be sent to other users directly in the future; (ii) User competition model: Multiple users download the video data from the same server with the limited resource, and the server optimizes the resource for each user; (iii) User cooperation model: Similar to our model, users cooperate with each other to download video data. The difference is that in those models, only one user requests the video data, while all other users are helpers; in our model, all users request the different video data.


%The  {Dynamic Adaptive Video Streaming over HTTP (DASH)} is a standard for adaptive bitrate video streaming \cite{dash}, supporting flexible stream switching, multiple-base URLs and multilayer coded streams\cite{standard}. Recently, technical specifications (such as 3GPP Rel.~9 \cite{3GPPr9} and OIPF  Rel.~2 \cite{OIPFr2}) and applications (such as HbbTV\cite{HbbTV}) have adopted DASH to achieve HTTP adaptive streaming.


%Dynamic Adaptive Streaming over HTTP (DASH) is a new standard for adaptive bitrate video streaming, and has been adopted by 3GPP Release 10 for streaming multimedia over wireless networks.
%Readers can refer to \cite{standard} and \cite{mpeg-dash} for the detailed description on DASH, including model structure, data format, and other features.


%\com{Seems that there are three methods:
%- Buffer based
%-Channel prediction based
%- Hybrid}



Prior works on ABR streaming mainly focused on the bitrate adaptation of a \emph{single user} (see \cite{b4} for a comprehensive discussion), including the {buffer-based} method \cite{b1}, the {channel prediction-based} method \cite{b6}, and the {hybrid} buffer- and prediction-based method \cite{b2, b8,b5,b10,b7}. 
Specifically,
In \cite{b1}, Huang \emph{et al.}~changed the video bitrate by a mapping from the current buffer level to reference bitrate.
In \cite{b6}, Li \emph{et al.}~choosed the segment bitrate based on the predicted channel capacity. 
%This work also considered the fair bandwidth sharing among multiple users.
Among the hybrid scheduling methods, Hao \emph{et al.}~in \cite{b2} proposed  a  geo-predictive streaming system for predicting the  available network bandwidth in different locations and constructing the bandwidth map, which is used for the bitrate adaptation with the buffer size.



%%Part 2
%%One of the key problems in DASH is the scheduling of segment downloading.
%Prior works on the scheduling method in DASH mainly focused on the single-user model.
%%\textit{Buffer-based scheduling} and \textit{channel prediction based scheduling} are two main methods used in DASH.
%In general, there are three types of scheduling methods  \cite{b4}: (i) \emph{buffer based} method  (e.g.,\cite{b1}), (ii) \emph{channel prediction based} method (e.g., \cite{b6}), and (iii)  \emph{hybrid} method (e.g., \cite{b2, b8,b5,b9,b10,b7}), which combines both the  buffer based and channel prediction based ideas.
%In \cite{b1}, Huang \emph{et al.}~changed the video bitrate by a mapping from the current buffer level to reference bitrate.
%In \cite{b6}, Li \emph{et al.}~proposed a channel prediction method, and choosed the segment bitrate based on the predicted channel capacity.
%%This work also considered the fair bandwidth sharing among multiple users.
%Among the hybrid scheduling methods, Hao \emph{et al.}~in \cite{b2} proposed   geo-predictive streaming system for predicting the  available network bandwidth in different locations and constructing the bandwidth map, which is used for the bitrate adaptation with the buffer size.
%%Tian \emph{et al.}~in \cite{b9} proposed a PI controller with input  {reference buffer size}, feedback  {current buffer size}, and disturbance  {predicted/actual channel capacity}, aiming at maintaining the buffer occupancy  by properly selecting the bitrate according to the current buffer level and the predicted channel capcity.


Some recent works extended the basic single-user model to more advanced ones, such as the  multi-link model \cite{c7}, the multi-server model \cite{b9}, and the P2P model \cite{c1,c2,c3,YunTang2006,PooKuanHoong2008}, \rev{and studied the associated incentive issues.}
Specifically,
In \cite{c7}, Xing \emph{et al.}~considered the scenario where a user  connects to server via multiple links (e.g. 3G and WiFi) to reduce the user energy cost and increase the user utility.
However, the above work did not consider the cooperation of multiple   users.
In \cite{b9}, Tian \emph{et al.}~considered the multi-server model, where users download video from multiple servers to reduce the server load.
In \cite{c1,c2,c3,YunTang2006,PooKuanHoong2008}, researchers constructed adaptive streaming models on P2P systems to reduce the server load, and studied related technical and economic issues for promoting the user cooperation in the P2P streaming.
\revv{There are several key differences  between our proposed crowdsourced streaming model and the above multi-server \cite{b9} and P2P \cite{c1,c2,c3,YunTang2006,PooKuanHoong2008} streaming models.
In the multi-server and P2P streaming models,
each video segment has multiple copies resided on
multiple servers or multiple user devices (peers).
Video users can download a video segment either from a server or from a user peer, via his own wireless access link.
Hence, the key design purpose of such multi-server or P2P model is
\emph{to reduce the load of the video server}.
In our crowdsourced streaming model, however, each video segment has a unique copy residing on the video server, and users can download a video segment (from the   server) either via his own wireless
access link or a neighbor's access link.
Hence, the key design purpose of such a crowdsource streaming model is \emph{to reduce the uncertainty or improve the efficiency of user's wireless access link}.}~~~~~~~~~~~~~~~~


%Part 3
%Some recent researches extended the basic single-user  model to more advanced ones, such as the P2P model \cite{c1,c2,c3}, the multi-server model \cite{b9}, and the  multi-link model \cite{c7}.
%Specifically, in \cite{c1,c2,c3}, researchers constructed DASH models on P2P systems to reduce the load of video server.
%%Clients can download segments from other peers who have already buffered the required segments.
%In \cite{b9}, Tian \emph{et al.} considered the multiple server scenario, where clients download from multiple servers to reduce the server load.
%In \cite{c7}, Xing \emph{et al.} considered the scenario where a client connects to network via multiple links (e.g. 3G and WiFi), to reduce the client cost and maximize the client utility.
%However, none of the above work considered the cooperation of clients in video scheduling.
%However, none of the above work considered the scenario where neighbouring clients cooperate with each other to schedule segments, so as to reduce the
%impact of wireless channel fluctuation.

Moreover, there is also a growing interest in exploiting the multi-user adaptive video streaming scenarios \cite{c5, c6, multiuser-dash-1, multiuser-dash-2, multiuser-dash-3}.
Specifically, in \cite{c5} and \cite{c6}, researchers considered the user cooperation in mobile video streaming, and proposed models to aggregate the bandwidth of a mobile video user and its neighbours.
%Once a single client has video streaming requirement, some neighbour users (including himself) download and forward the required segments to the client.
%A centric task manager is responsible for the segment scheduling.
%Clients in this paper can either connect to both links or connect to WiFi only, to efficiently utilize the network resources.
However, these models focused on the simple one-to-many cooperation scenario with a single video user and many helpers. We consider a more general many-to-many cooperation framework with multiple video users, where each user acts as a video player and a helper simultaneously.
In \cite{multiuser-dash-1}, Pu \emph{et al.} proposed a rate adaptation algorithm for optimizing the adaptive streaming across multiple mobile users, but they did not consider the individual characteristics of different users.
In \cite{multiuser-dash-2}, Georgopoulos \emph{et al.} studied multiuser streaming in a home networking scenario, but they did not consider the important network characteristics such as the
transmission rates.
In \cite{multiuser-dash-3}, El Essaili \emph{et al.} studied the mobile network potential for enhancing the user QoE in multiuser DASH over LTE cellular networks, and proposed the joint
optimization of transmission and bitrate of the mobile DASH users considering their buffer levels.
However, they neither considered the performance bound, nor the online algorithm. 
In this work, we study the  multi-user cooperative video streaming (both online and offline) by using the crowdsourced UPN technology.

%We focus on the interactions among all users in a crowdsourced model.

%\revvv{The idea of using network crowdsourcing to reduce cellular energy consumption has been studied by Nicutar \emph{et al.} in \cite{energy-new} (and the references therein), which indicates that lightly loaded cellular links consume almost as much power as fully loaded ones.
%Hence, by crowdsourcing the cellular links of nearby mobile users (via WiFi or Bluetooth) and consolidating   users' traffic onto a subset of cellular links, the total energy consumption can be effectively reduced.
%However, the above work (and the references therein) considered only the energy issue, without considering the unique feature of  video streaming and the optimal scheduling of multi-user streaming.
%To our best knowledge, this is the first work that using the network crowdsourcing technology to optimize a multi-user video streaming system.}




==> section6-online.tex <==
%!TEX root = DASH_Main_JSAC.tex
%SourceDoc DASH_Main_JSAC.tex



\section{Online Scheduling Algorithms}
\label{sec:main2}

In   previous sections, we have analyzed the theoretical performance upperbound of the proposed crowdsourced system, which is achievable only in an ideal scenario with the complete network information.
In practice, however, network information changes randomly over time. Hence, it is difficult  to  obtain the future and global network information.~~~~~~~~

In this section, we study the practical scenario where the future and global network information is not available.
We propose an online scheduling algorithm based on the Lyapunov optimization framework [30], which relies only on the current local  network information and the scheduling history, while not on any future or global network information.
%For performance comparison, we also review several typical
%online scheduling algorithms in the existing literature.



\subsection{Online vs Offline}

We first discuss the key difference between online scheduling and offline scheduling.
In the offline scheduling (Section \ref{sec:formulation}), the segment downloading sequences of all users for all time are determined in advance, through, for example, the offline social welfare maximization problem \eqref{eq:swm}, together with the complete network information.
In the online scheduling, however, each user makes the download scheduling decision  (regarding the next segment to be downloaded) in real time, e.g., at the time when he completes a previous segment downloading.

In our proposed crowdsourced system, such a real time downloading decision mainly includes whose segment to be downloaded, and at which bitrate level.
The decision may depend on different criteria such as
the real time user buffer levels (e.g., in \cite{b1}),
the channel bandwidth or throughput predictions (e.g., in \cite{b6}),
and other specific objective functions (e.g.,
Lyapunov drift-plus-penalty described below).~~~~




\subsection{Lyapunov-Based Online Scheduling}

%Key idea: Whenever completing a segment downloading, a user will choose the next segment according to the Lyapunov optimization method.

Lyapunov optimization [30] is a widely used technique for
solving stochastic optimization problems with time average
constraints.
In our model, an implicit time average constraint is that
the average segment arriving rate should be same as the video playback rate in term of segment.\scfootnote{For example, for a video with 2-second segment, the playback rate in term of segment is 0.5 (segments per second).}
%\scfootnote{{The data downloading rate is the product of segment arriving rate and the average bitrate of each segment.}}
%\com{How to define this? This depends on the downloading policy and the channel capacities?
%If the channel capacities are small, then it is not possible to download fast enough.
%However, if the channel capacities are large, then it is possible to schedule the download properly such that this condition is satisfied (such as pause for some time before downloading the next segment)? }
\revh{If the video playback rate is smaller, then the downloaded segments will be frequently dropped due to the limited buffer size;
if the video playback rate is larger, then the rebuffering will frequently happen.
Both cases are not desirable in this system.}
To this end, we introduce the Lyapunov optimization technique to optimize the downloading scheduling  in an online manner.

Suppose that a user $n$ completes a segment downloading at time $t$, and needs to make the downloading decision regarding the next segment to be downloaded.
We denote such a decision  by $(u, z)$, where $u\in \N$ is the owner of the segment to be downloaded, and $z\in \{1,...,Z\}$ is the bitrate level of the segment to be downloaded.
Obviously, a feasible decision $(u,z)$ of user $n$ at time $t$  satisfies the following user encounter constraint: $e_{n,u}(t) = 1$.


For analytical convenience, we further denote $\buf_m (t) $ as the  buffer level  of each user $m$ at time $t$,
and denote $r_m $ as the bitrate of user $m$'s \emph{last received}  segment.  This information essentially captures the current network state and historical scheduling information  that can be observed.

\emph{1) \textbf{Objective Function:}}
Given a feasible decision $(u, z)$ of user $n$, the data volume to be downloaded is $R_u^z  \cdot \tseg_u$ (Mbit), and the \emph{estimated} downloading time is $\gamma_{u,z} \eq \frac{R_u^z  \cdot \tseg_u}{h_n(t)}$.\scfootnote{Here we use the current channel capacity $h_n(t)$ to approximate the capacity in a period of future time.
Note that the actual downloading time may be different from $\gamma_{u,z} $ due to the channel stochastics.}
%\com{The costs and utility defined before are in terms of the whole time period [0,T]. However, here we are defining costs and utility for a small time interval? Even during this small time interval, there can be multiple segments downloaded by multiple users for multiple users. Hence we are focusing on the cost and utility of a single segment downloading? Need to explain clearly. }
\revv{The total energy consumption of user $n$ (\emph{for this particular   downloading operation}) and user $n$ (for playing the downloaded segment)  is:}
\begin{equation*}
 \begin{aligned}
&  \Cost_n(u,z)  =    \Costc_n + \Costw_n + \Costxx_u
 \\
&
\textstyle
=\left( \cct_n \cdot \gamma_{u,z} +
\ccv_n \cdot  R_u^z  \cdot \tseg_u \right)  +
 \textstyle \cwv_n \cdot  R_u^z  \cdot \tseg_u \cdot \mathbf{1}(u\neq n)
 + 
 \left( \cxxt_u \cdot \tseg_u +
\cxxv_u \cdot  R_u^z  \cdot \tseg_u \right)
  ;
\end{aligned}
\end{equation*}

The utility of segment receiver $u$ \emph{on this particular segment} is
\begin{equation*}
\begin{aligned}
 \Ut_u(u,z) &  = \Va_u- \Lossdeg_u- \Lossrebuf_u
 \\
&
 \textstyle
 = g_u(R_u^z) \cdot  \tseg_u
 -
  \ld_u  \cdot [ r_u  - R_u^z ]^+
  -
   \lr_u   \cdot \left[  \gamma_{u,z}   -  \buf_u (t)  \right]^+;
\end{aligned}
\end{equation*}

The utility of other user $m $ (other than $u$) due to this operation is
\begin{equation*}
 \textstyle  \Ut_m(u,z)  = \Lossrebuf_m=
-    \lr_m \cdot  \left[  \gamma_{u,z}  -  \buf_m (t) \right ]^+ , ~~
\end{equation*}
which only includes the potential rebuffering loss.



Therefore, the total   payoff generated under $(u, z)$ is
\begin{equation}\label{eq:obj}
\Pay(u, z) \eq  \sumM \Ut_m(u,z)  - \Cost_n(u,z).
\end{equation}

%where
%$ \Va_u  $ is the achieved value of user $u$,
%$ \Lossdeg_u  $ is the  quality degrade loss of user $u$,
%$\Lossrebuf_u  $ is the \emph{estimated} rebuffering loss of user $u$,
%$\Costc_n  $
%is the energy cost of user $n$ on cellular link,
%and
%$\Costw_n =   $
%is  the   energy cost of user $n$ on WiFi link (when downloading for others).
%Here, $\frac{R_u^z \cdot \tseg_u}{h_n(t)}  $ is the \emph{estimated} downloading time, as we use the current channel capacity $h_n(t)$ to approximate the capacity in a period of future time.
%Note that the actual downloading time may be different from $\frac{R_u^z \cdot \tseg_u}{h_n(t)}  $ due to the changing of  channel capacity.



\emph{2) \textbf{Lyapunov Drift:}}
Following the Lyapunov framework, we   define a modified Lyapunov function:
 \begin{equation}
 J(t) \eq \frac{1}{2}   \sumM \left[\Q_m -   \buf_m (t) \right] ^2.
\end{equation}
The \emph{Lyapunov drift} is  the change of Lyapunov function (from one decision-making time to the next), i.e.,
 \begin{equation} \label{eq:drift}
\begin{aligned}
\Delta(t) & \eq  J(t +  \gamma_{u,z}) - J(t),
\\
& = \frac{1}{2} \sumM \left( \left[\Q_m -   \buf_m (t + \gamma_{u,z}) \right]^2 -   \left[\Q_m -   \buf_m (t) \right]^2 \right),
\end{aligned}
\end{equation}
where $\buf_m (t + \gamma_{u,z})$ is the estimated buffer level of user $m$ at time $t + \gamma_{u,z}$
(i.e., the next decision-making time of user $n$).
For the segment receiver  $u$,  the estimated buffer level is:
$$
\buf_u (t + \gamma_{u,z}) = \min\{\Q_u,\ [\buf_u (t) - \gamma_{u,z}]^+ +  \tseg_u \};
$$
For other user $m $ (other than $u$), the estimated buffer level is:
$$
\buf_m (t + \gamma_{u,z}) = [\buf_m (t) - \gamma_{u,z}]^+  ;
$$



\emph{3) \textbf{Online Scheduling Algorithm:}}
By the Lyapunov optimization theorem, to stabilize the system while optimizing the objective, we can use such a scheduling policy that greedily minimizes \emph{drift-plus-penalty}:
 \begin{equation} \label{eq:drift-penalty}
\Phi(t) \eq  \Delta(t) - \lambda \cdot  \Pay(u, z),
\end{equation}
where  the negative payoff $(-\Pay(u, z))$ is viewed
as the penalty incurred at time $t$, and  $\lambda \geq 0$ is a control parameter.
It is important to note that the buffer levels (appearing in $\Delta(t)$) serve as regulation factors, such that the user
with a larger idle buffer can be more likely to be scheduled (hence
reducing the possibility of rebuffering). 
This term is different from the rebuffering loss in (\ref{eq:loss-rebuf}), which is the actually realized loss when a rebuffering event
actually happens.
%\com{Minimizing negative payoff (-P(u,z)) is equivalent of maximizing the payoff P)u,z)? }
 


Based on the above   analysis, we now design an
on-line algorithm that aims at minimizing the drift-plus-penalty
\eqref{eq:drift-penalty} in each decision-making time.
We present the detailed algorithm in Algorithm \ref{algo:Lya}.
Note that a user may decide \emph{not} to
download any segment at a decision-making time, when, for example, all buffers are full and cannot afford one more segment.
In this case, the user will wait for a certain time and then trigger decision-making event again.
Hence, a decision-making time can be either the time that a user   completes a segment downloading, or the time that a user  is triggered by the waiting timer.

\revv{To implement Algorithm \ref{algo:Lya} in practice, nearby users need to exchange certain information in order to make the downloading decision as well as to avoid the redundant downloading of the same segment. 
Two key processes are as follows. 
First, users periodically broadcast their buffer levels to neighbors through WiFi, 
such that each user can compute the accurate buffer levels of all neighbors at any time for making the downloading decision. 
Second, when a user decides to download video for another user, he queries the latter (who knows the detailed information regarding his received and scheduled segments) for the detailed information (e.g., url) of the segment to be downloaded. This can avoid the redundant downloading of the same segment for another user.}


\begin{algorithm}[t]
\label{algo:Lya}
\caption{Lyapunov-based Online Scheduling}
\DontPrintSemicolon
%\BlankLine
%\emph{The economic interaction of master $m$ with the database and the end-users}\;
\While{at each decision-making time $t$}
{
\If{$\buf_n(t) + \tseg_n > \Q_n , \forall n\in \N$}
{
/* \emph{no buffer can afford one more segment}  */
\\
Wait for $T_w =  \min_{n\in\N} (\buf_n(t) + \tseg_n - \Q_n)$  seconds;
}
\Else
{
Download a segment of bitrate level $z^*$  for user $u^*$:
\\
$ ~~~~~
(u^*, z^*) = \arg \min_{u , z  } \  \Phi(t) \eq  \Delta(t) - \lambda \cdot  \Pay(u, z)
$
}
}
\end{algorithm}


\emph{4) \textbf{Performance Analysis:}}
Now we analyze the performance of Algorithm \ref{algo:Lya}.
Let $t_{[k]}$ denote the $k$-th decision-making time (counting  all users), and let $\Pay_{[k]}$ denote the associated payoff achieved in the $k$-th download operation.
Then, the total social welfare during the entire time horizon $[0,T]$ generated by Algorithm \ref{algo:Lya} can be written as:
$$
\textstyle
\SWi_{(\btseg)} = \sum_{t_{[k]} \leq T} \Pay_{[k]}.
$$
By the Lyapunov optimization theorem  (Theorem 4.2 in \cite{lya}), we obtain the following gap for $\SWi_{(\btseg)}$ and $\SWo_{(\btseg)} $, i.e., the theoretical performance upperbound.
\begin{theorem} \label{theorem:2}
$$
\lim_{T \rightarrow \infty}
 \
\mathrm{E} \left[ \SWi_{(\btseg)} \right]
 \geq
\mathrm{E} \left[ \SWo_{(\btseg)}  \right] - \frac{B}{\lambda},
$$
where $\mathrm{E}[.]$ is expectation, and $B$ is a positive constant.
\end{theorem}

Theorem \ref{theorem:2} shows that Algorithm \ref{algo:Lya} converges to the theoretical performance upperbound  $\SWo_{(\btseg)}$  asymptotically, with a controllable approximation error bound $O(\frac{1}{\lambda})$.
However, this theorem does not directly help us calculate the \emph{actual gap} between $\SWi_{(\btseg)}$ and $\SWo_{(\btseg)} $ in a particular experimental scenario, as we have a finite value of $T$ in practice.
%due to the finite $T$ as well as the difficulty in computing the theoretical $\SWo_{(\btseg)} $.
To this end, we propose another approach based on Theorem 1 for the practical calculation of the actual gap, i.e.,
$$
\big| \SWo_{(\btseg)} - \SWi_{(\btseg)} \big|
\leq
\big| \SWx_{(\btseg' \rightarrow \mathbf{0})} -\SWi_{(\btseg)} \big|.
$$
Note that $ \SWx_{(\btseg' \rightarrow \mathbf{0})}$ is the solution of the integer programming problem (\ref{eq:swm-slot}), and can be easily computed in a practical experiment after collecting the complete network information.
In our experiments, the average gap between $\SWi_{(\btseg)}$ and $\SWx_{(\btseg' \rightarrow \mathbf{0})}$ is smaller than $3\%$.

%\subsection{Buffer-Based Online Scheduling in \cite{xx}}
%
%
%\subsection{Channel Prediction-Based Online Scheduling in \cite{xx}}
%
%Key idea: Whenever completing a segment downloading, a user will choose the next segment only based on the buffer sizes of all encountering users.


%
%%
%%
%\begin{figure*}[t]
%  \centering
%  \includegraphics[height=1.55in]{sim/multiple-bitrateline}
%  ~~~~
%  \includegraphics[height=1.55in]{sim/multiple-swline}
%  ~~~~
%  \includegraphics[height=1.55in]{sim/multiple-swbar}
%  \caption{(a) Average video  Bitrate, (b) Social Welfare, (c) Average Social Welfare, in Two-User Case with Simulation Data.}
%  \label{fig:multiple}
%\end{figure*}


==> section7-experiment.tex <==
%!TEX root = DASH_Main_CISS_new.tex
%SourceDoc DASH_Main_CISS_new.tex


\section{Experiments and Performance}\label{sec:simulation}

%We will design experiments (or simulations, or numerical study) here ... \\
%
%We will evaluate the performance of the proposed online scheduling algorithms ... \\
%
%We will also compare the online scheduling algorithms with the     algorithms  in the existing literature ...



\begin{figure}[t]
  \centering
  \includegraphics[height=2in]{sim/fig-measured-throughput}
  \vspace{-3mm}
  \caption{Measured Throughputs.}
  \label{fig:measured-th}
  \vspace{-3mm}
\end{figure}


% 2.55 2.46 0.44 0.88
\begin{figure*}[t]
\vspace{-4mm}
   \centering
  \includegraphics[width=.23\textwidth]{sim/aa-single-bitrate}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-single-sw}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-single-avgbitrate}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-single-avgsw}
  \vspace{-1mm}
\\
~~~~~~~~
~~~~~
(a)
~~~~~~
~~~~~~~~
~~~~~~~~
~~~~~~~~
(b)
~~~~~
~~~~~~~~
~~~~~~~~
~~~~~~~~
(c)
~~~~~~~~
~~~~~
~~~~~~~~
~~~~~~~~
(d)
~~~~~~~~
~~
\vspace{-3mm}
  \caption{(a) Average Bitrate in Each Experiment, (b) Social Welfare in Each Experiment, (c) Average Bitrate in 1000 Experiments, (d) Average Social Welfare  in 1000 Experiments.
  (Red: Offline-Benchmark,
  Blue:  Lyapunov-Online,
  Green:   Prediction-Online,
  Pink:  Buffer-Online)}
  \label{fig:single-real}
\vspace{-3mm}
\end{figure*}

\subsection{Experiment Setting}

 {\emph{1) \textbf{Datasets:}}
To evaluate the realistic performance of our proposed crowdsourced system, we conduct experiments using real data traces from two datasets: ISF\scfootnote{ISF is provided by a non-profit organization named ``Ile Sans Fil'' in Canada, and is open source (available at CRAWDAD   \cite{data1}, the Community Resource for Archiving Wireless Data At Dartmouth).} and NWF\scfootnote{NWF is obtained from a recent wireless service provider called NextWiFi in China \cite{data2}.}.
Both datasets trace the user access sessions at a set of WiFi hotspots in different countries during a long period of time (3 years for ISF and 5 months for NWF).
Each session records the information of one access (of a particular user at a particular hotspot), including user id, hotspot id, login and logout time, incoming and outgoing traffic volumes, etc.
%\com{In submission stage, should the name of company NextWIFI  be anonymous for double blind review ?}
These datasets represent two different (hotspot-based) mobility scenarios:  Users encounter more frequently in NWF, while the duration of each encounter is larger in ISF.}
%\rev{The average user encounter time in the ISF dataset is larger than that in the XXXX one;
%the average number of users encountered by a particular user in ??? is smaller than that in ???}




 {To simulate the video watching behaviours of mobile users and the real cellular link throughputs for video streaming, we use the video viewing session logs obtained from BestTV \cite{data3}, one of the largest OTT (Over The Top) video service providers in China.
%\com{In submission stage, should the name of company BesTV be anonymous for double blind review ?}
Every session records the information of one video playing (of a particular mobile user towards a particular video), containing the detailed records of all segments, each including the user id, video id, segment id (playback index), segment length, resolution, bitrate, downloading time, etc.
There are 5 different bitrate levels (for mobile users) in this dataset: $\{0.2, 0.4, 0.7, 1.3, 2.3\}$Mbps, corresponding to the lowest to the highest video resolutions, respectively.
%has several   thousands of records, each of which represents a 10-second video chunk, \com{here, each chunk is 10 seconds,  while in 3.2 we mentioned 2 seconds, how about the chunk length in our experiment ?} containing the following information: user id (anonymized), ip address,  device information, chunk size, downloading time, video id, and  bitrate (identified by S1, S2, S3, S4, and S5, corresponding to 0.2, 0.4, 0.7, 1.3, 2.3Mbps).
Based on the segment length, bitrate, and downloading time, we can calculate the measured end-to-end link throughput for each
segment downloading.
We use this measured throughput to approximate the cellular link capacity in our experiments.
Fig.~\ref{fig:measured-th}  illustrates the probability distribution of the measured throughput, which shows that $10\%$ users experience a throughput lower than $0.7$Mbps, $40\%$ users experience a throughput lower than $1.3$Mbps, $50\%$ users experience a throughput lower than $2.5$Mbps, and $85\%$ users experience a throughput lower than $5.0$Mbps.}


Moreover, the energy consumption factors
are chosen according to the real measurement provided in the existing
literature \cite{energy,smartphone-energy}.


%
%
%\begin{figure*}[t]
%  \centering
%  \includegraphics[height=1.6in]{sim/single-real-bitrateline}
%  ~~~~
%  \includegraphics[height=1.6in]{sim/single-real-swline}
%  ~~~~
%  \includegraphics[height=1.6in]{sim/single-real-swbar}
%  \caption{(a)  Bitrate, (b) Social Welfare, (c) Average Social Welfare, in Single-User Case with Real Data.
%  (Red: Benchmark-Offline,
%  Blue:  Lyapunov-Online, Pink:  Buffer-Online, Green:   Prediction-Online)}
%  \label{fig:single-real}
%\end{figure*}





{\emph{2) \textbf{Existing Online Algorithms:}}
To evaluate the performance of our proposed Lyapunov-based online algorithm, we also perform simulations using the following two online algorithms in the literature: Buffer-based algorithm in \cite{b1} and Channel Prediction-based algorithm in \cite{b6}.\scfootnote{We have tried a lot of existing algorithms, and the ones in \cite{b1} and \cite{b6}  achieve the best performance (among all existing algorithms) in our experiments.}
Specifically, the buffer-based algorithm \cite{b1} introduces a linear mapping between buffer and bitrate, and selects the next segment bitrate based on the current buffer level: \emph{a higher buffer level is mapped to a higher bitrate}.
%This paper also considered constant bitrate mapping within \textit{reservoir} and \textit{upper reservoir}(i.e. low and high buffer size respectively), aiming at reducing the rebuffering rate and capacity waste.
%Bandwidth Based Method
The channel prediction-based algorithm \cite{b6} proposes a channel prediction method, and chooses the next segment bitrate based on the predicted channel capacity: \emph{choosing the highest bitrate that can be supported by the predicted channel capacity}.
%, which is the highest bitrate that supported by the predicted channel capacity. The channel prediction process considered both previous predicted channel capacity and prediction error. The performance of this algorithm also depends on coefficient selection. % In our simulation, we used the coefficient that provided in reference \cite{b6}.

Note that both algorithms in \cite{b1}  and \cite{b6}  were designed for the single-user scenario, and considered only the bitrate adaptation.
In the multi-user scenario, we need to consider both   bitrate adaptation and   segment owner selection (i.e., whose segment to be downloaded) as discussed in Section \ref{sec:main2}.
To this end, we introduce the following segment owner selection policy for these two algorithms in the multi-user scenario:
\emph{Each user $n$ will choose to download the next segment for  another user $u \neq n$, if and only if (i) $\buf_n \geq \delta_{\textsc{th}} \cdot \Q_n$, (ii) $ \buf_n -\buf_u \geq \Delta_{\textsc{th}} $, and (iii) $ \buf_u = \min_{m\in\N} \buf_m $.}
Intuitively, user $n$ will choose to help the user with the lowest buffer level, if his own buffer level is higher than a ratio threshold $\delta_{\textsc{th}}$ and meanwhile is higher than the lowest buffer level by  a threshold $\Delta_{\textsc{th}}$. In our experiments, we will try different values of $\delta_{\textsc{th}} $ and $\Delta_{\textsc{th}}  $, and choose the best ones.}



\subsection{Single-User Case}



We first construct experiments for the single-user scenario (i.e., non-cooperative scenario), where the user plays a high-resolution video (bitrate $2.3$Mbps). The total video length is 500 seconds,  the segment length is 2 seconds, and the maximum  buffer length at the user's device is 40 seconds.
 {We use these experiments to illustrate the performance gap of our proposed Lyapunov-based online algorithm to the theoretical performance bound.
We also use these experiments to compare the bitrate adaptation performance of our proposed algorithm with the existing online algorithms.}

%\com{maybe this case would confuse reviewer, why we compare the performance in single user case?
%Here lack of some analysis about why online algorithm outperforms others in single user case. Does it mean we propose a better rate selection approach ? }
%\com{it's too lager for video player.
%how does buffer length impact performance in our experiments ?}

Figure \ref{fig:single-real} shows the average bitrate and social welfare under different average link capacities (extracted from the measured link throughput traces).
Red curve/bar denotes the theoretical upperbound (benchmark), Blue curve/bar denotes the proposed Lyapunov-based online algorithm,
Green curve/bar denotes the  channel prediction-based algorithm in \cite{b6},
and Pink curve/bar denotes the
buffer-based  algorithm in \cite{b1}.
Each point in subfigures (a) and  (b) denotes the average bitrate and   social welfare generated in one experiment (corresponding to a particular choice of data trace), respectively.
Subfigures (c) and (d) shows the average bitrate and average social welfare in 1000 experiments under different average link capacity ranges.
For example, in the first bar group, we calculate the average bitrate and average social welfare achieved in all experiments with an average link capacity below 0.7Mbps.


We can see from (a) and (c) that our proposed algorithm (Blue) achieves
an average bitrate   higher than other two  algorithms (with an average bitrate increase of $5\%\sim30\%$), and is very close to the offline benchmark (Red).
We can further see from (b) and (d) that our proposed algorithm achieves an average social welfare higher than other two algorithms (with an average gain of $10\% \sim 40\%$), and is very close to the theoretical upperbound (with an average gap less than $3\%$).
Moreover, the social welfare gain decreases with the maximum link capacity.
This is because with a larger link capacity, all algorithms approach to the upperbound, hence their differences become less significant.

 {The above experiments demonstrate
that the bitrate adaptation mechanism in our   algorithm is better than those in \cite{b1} and \cite{b6}. By Theorem 2,
our algorithm asymptotically
converges to the theoretical performance upperbound (with
a controllable gap), while the other two algorithms represent some reasonable heuristics without a theoretical performance guarantee.}
%Since there is no impact of segment owner selection in the single-user case, these experiments show that the bitrate adaptation in our proposed algorithm outperforms the buffer-based and the prediction-based bitrate adaptation in \cite{b1} and \cite{b6}.}
%In fact, by the Lyapunov optermization theory, our algorithm provably converges to the theoretical performance upperbound (with a controllable gap), while the other two algorithms just operate in a plausible way.

%
%\begin{figure*}[t]
%  \centering
%  \includegraphics[height=1.6in]{sim/multiple-real-bitrateline}
%  ~~~~
%  \includegraphics[height=1.6in]{sim/multiple-real-swline}
%  ~~~~
%  \includegraphics[height=1.6in]{sim/multiple-real-swbar}
%  \caption{(a)    Bitrate, (b) Social Welfare, (c) Average Social Welfare, in Two-User Case with Real Data under Full Encounter.
%  (Blue:  Lyapunov-Online, Pink:  Buffer-Online, Green:   Prediction-Online)}
%  \label{fig:multiple-real}
%\end{figure*}
%
%
%
%\begin{figure*}[t]
%  \centering
%  \includegraphics[height=1.6in]{sim/many-real-swline}
%  ~~~~
%  \includegraphics[height=1.6in]{sim/many-real-swbar}
%  \caption{(a) Social Welfare (5 Users), (b) Average Social Welfare, in Real Multi-User Scenario.
%  (Blue:  Lyapunov-Online, Pink:  Buffer-Online, Green:   Prediction-Online)}
%  \label{fig:many-real}
%\end{figure*}



%Figure \ref{fig:single-real} shows the average bitrate and social welfare under realistic link capacities (extracted from real data traces).
%Here the average link capacity in real data traces ranges from  $0.7$Mbps  to $10$Mbps.
%Similarly, we can see that our proposed algorithm outperform the other two algorithms in terms of the average bitrate and social welfare.
%However, the performance increase becomes less significant in this case (increasing the average bitrate by $10\% \sim  20\%$ and the social welfare  by $5\% \sim 10\%$).
%Similarly, we can see from (a) that our proposed algorithm achieves
%an average bitrate higher than other two  algorithm (with an average bitrate increase of $10\% \sim 20\%$).
%We can further see from (c) that our proposed algorithm achieve a social welfare higher than other two algorithms (with an average gain of  $5\% \sim 10\%$), and close to the theoretical upperbound (with an average loss less than $3\%$).
%Here, the performance gain  is smaller than that in Figure \ref{fig:single}.
% The reason is that all three online algorithms achieve very good performances due to the large link capacity,  hence their differences are not significant.

%\com{we need more discussions and analysis about the results, not only show the results }
%
%\com{Do we have the results in the case of multiple user with different download task, some watch video, some browse web site ?}


%\com{The following simulations are in processing ... }

\subsection{Multiple-User Case}

\begin{figure*}[t]
 \vspace{-3mm}
 \centering
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgbitrate-100}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgbitrate-60}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgbitrate-20}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgbitrate-increase}
  \vspace{-1mm}
\\
~~~~~~~~
~~~~~
(a)
~~~~~~
~~~~~~~~
~~~~~~~~
~~~~~~~~
(b)
~~~~~
~~~~~~~~
~~~~~~~~
~~~~~~~~
(c)
~~~~~~~~
~~~~~
~~~~~~~~
~~~~~~~~
(d)
~~~~~~~~
~~
\vspace{-3mm}
  \caption{(a) Average Bitrate with 100\% Video Users, (b) Average Bitrate with 60\% Video Users, (c) Average Bitrate with 20\% Video Users, (d) Average Bitrate Increase under the Lyapunonv-based Algorithm.}
  \label{fig:multiple-bitrate}
 \vspace{-3mm}
\end{figure*}

%
%%
%\begin{figure}[t]
%  \centering
%  \includegraphics[height=2.4in]{sim/multiple-cooperation-gain}
%  \caption{Cooperation Gain in Two-User Case with Simulation Data.}
%  \label{fig:multiple}
%\end{figure}
%
%
%\emph{1) \textbf{Cooperation Gain:}}
%We illustrate the cooperation gain achieved by the proposed crowdsourced cooperative network.
%To better illustrate such a cooperation gain, we provide a set of toy network scenarios with two users \{1, 2\}, where user 1's average link capacity changes from 0.5Mbps to 6Mbps, and user 2's average link capacity is zero (e.g., when he has no feasible Internet connection).
%In the first scenario (Blue bar), both users want to play a high-resolution video (bitrate 2.3Mbps);
%In the second scenario (Green bar), user 2 wants to play a high-resolution video, and user 1  wants to play a middle-resolution video (bitrate 0.7Mbps);
%In the third scenario (Red bar), user 2 wants to play a high-resolution video, and user 1  wants to play a low-resolution video (bitrate 0.2Mbps).
%In each bar group, the hollow bar denotes the maximum social welfare (i.e., the theoretical upperbound) in the crowdsourced system, and the corresponding solid bar denotes the maximum social welfare  in the non-cooperative system.
%We can see that in the above scenarios, the cooperation gain can be up to $200\%$ (the last red bar).
%In fact, depending on different scenarios, such a cooperation gain can be infinitely large, e.g.,  in the scenario where the users with capacity have no service and the users without capacity have video service.
%
%
 Now we perform experiments for the multi-user scenario, where some users play  videos (called video users), while others remain idle and can potentially help the encountered video users.
For simplicity, we assume that all video users play the high-resolution videos (bitrate $2.3$Mbps).
The video configuration (such as video length, segment length, and buffer size) is same as those in the single-user case.
We use these multi-user experiments to illustrate both the cooperation gain of the proposed crowdsourced system and the performance gain of the proposed algorithm.






In the following experiments, we consider a total of 50 users and randomly choose a subset of users as video users.
We consider different network conditions, characterized by the \emph{range} of the average link capacity.
%We consider 5 levels of different network conditions, corresponding to capacity ranges of $[0, 0.7]$Mbps, $[0, 1.3]$Mbps, $[0, 2.5]$Mbps, $[0, 5.0]$Mbps, and $[0, 8.0]$Mbps, respectively.
For example, a bad network condition corresponds to a range $[0, 0.7]$Mbps, under which each user will be randomly assigned by a real data trace with an average link capacity smaller than $0.7$Mbps.

\emph{1) \textbf{Average Bitrate:}}
Figure \ref{fig:multiple-bitrate} shows the average bitrates with different percentages of video users under different network conditions.
For each video user percentage and network condition, we perform experiments with the three algorithms under ISF and NWF mobility traces, corresponding to different encountering scenarios (hence different cooperation probabilities).
To fully characterize the cooperation gain, we also run the algorithms under two benchmark encountering scenarios: (i) a full cooperation scenario, where all users are always encountered with each other, and (ii) a non-cooperative scenario, where none of users are encountered.
Sugfigures (a) to (c) show the average bitrates with $100\%$, $60\%$, and $20\%$ video users, respectively.
As illustrated in (a), the solid bar denotes the average bitrate under the non-cooperative scenario, and the hollow bar denotes the average bitrate under the full cooperation, in which the first (higher) line denotes the average bitrate under ISF (with a higher encountering probability) and the second (lower) line denotes the average bitrate under NWF (with a lower encountering probability).
Subfigure (d) shows the average bitrate \emph{increase} (i.e., the cooperation gain) with our proposed Lyapunov-based algorithm, comparing with  the achieved bitrate under the non-cooperative scenario.
The solid-dot lines denote the cooperation gain under the full cooperation scenario, the dash-square and dash-triangle lines denote the cooperation gain under the ISF and NWF, respectively.~~~~~~~~~~~~

From subfigure (a), we can see that when the percentage of (high-resolution) video users is very high (e.g., $100$\%), the  increase  of bitrate is very small under a low link capacity range (e.g., lower than $2.5$Mbps), as in this case all users are lack of capacity, hence nobody can help other users significantly.
Under a high link capacity range (e.g., $[0, 5]$Mbps and $[0, 8]$Mbps), the  increase  of bitrate becomes significant, as some users may have redundant capacities, hence can help others.
From subfigures (b) and (c), we can see that when the percentage of video users is low (e.g., $60\%$ or $20\%$), the increase of bitrate is significant under all network conditions, mainly due to the contributions of the idle users.

Subfigure (d) summarizes the increase of bitrate under our proposed algorithm.
We can see that with $100\%$ video users, the increase of bitrate continuously increases with the link capacity, as a larger capacity gives the video users more opportunities to obtain redundant capacity and help others.
With $20\%$ video users, however, the increase of bitrate continuously decreases with the link capacity, as a very small capacity already leads to a considerably high bitrate (due to the contributions of a large population of idle users), hence the increase of bitrate is more significant under a small capacity (as the benchmark bitrate is smaller).
With $60\%$ video users, the increase of bitrate first increases with the link capacity (due to a similar reason in the $100\%$ case), and then decreases with the link capacity (due to a similar reason in the $20\%$ case).
The maximum bitrate increase ratio under the full cooperation scenario can be up to $50\%\sim230\%$  with $20\%$ video users,
$35\%\sim60\%$ with $60\%$ video users, and $4\%\sim40\%$  with $100\%$ video users.
Moreover, the bitrate increase under the real data traces is bounded by the above maximum ration, and actually depends on the encountering probability. In our experiments, the bitrate increases under ISF and NWF can reach around $60\%$ and $40\%$ of the maximum bitrate increase, respectively.~~~~


\begin{figure*}[t]
\vspace{-4mm}
  \centering
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgsw-100}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgsw-60}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgsw-20}
  ~
  \includegraphics[width=.23\textwidth]{sim/aa-multiple-avgsw-increase}
  \vspace{-1mm}
\\
~~~~~~~~
~~~~~
(a)
~~~~~~
~~~~~~~~
~~~~~~~~
~~~~~~~~
(b)
~~~~~
~~~~~~~~
~~~~~~~~
~~~~~~~~
(c)
~~~~~~~~
~~~~~
~~~~~~~~
~~~~~~~~
(d)
~~~~~~~~
~~
\vspace{-3mm}
  \caption{(a)   Social Welfare with 100\% Video Users, (b)   Social Welfare with 60\% Video Users, (c)   Social Welfare with 20\% Video Users, (d)  Average Social Welfare Increase  under the Lyapunonv-based Algorithm.  }
  \label{fig:multiple-sw}
\vspace{-3mm}
\end{figure*}



\emph{2) \textbf{Social Welfare:}}
Figure \ref{fig:multiple-sw} shows the average social welfares and welfare gains with different percentages of video users under different network conditions.
The key informations and observations regarding the social welfare are similar as those regarding the average bitrate in Figure \ref{fig:multiple-bitrate}, hence we skip the detailed discussions and only present the results regarding the cooperation gain.
Specifically, using our proposed algorithm, the maximum social welfare increase ratio (under the full cooperation scenario) can be up to $20\%\sim40\%$ with $20\%$ video users,
$10\%\sim20\%$ with $60\%$ video users,
and
$5\%\sim15\%$ with $100\%$ video users.
The social welfare increase under ISF and NWF can reach $60\%$ and $40\%$ of the maximum welfare increase, respectively.~~~~~~~~~~~~~~~


%\revvv{\emph{3) \textbf{Energy Consumption:}}
% We now compare the energy consumptions under the full cooperation scenario and the non-cooperation scenario, both using our proposed Lyapunov-based online algorithm.
% Table \ref{energy:tbl} illustrate the ratio of energy consumptions (per bit of data downloading) under the full cooperation scenario and the non-cooperation scenario with different percentages of video users.
% We can see that using our proposed crowdsourced video streaming, under the full cooperation scenario, the average energy consumption reduction is $1\%\sim13\%$  with $100\%$ video users,
%$4\%\sim22\%$ with $60\%$ video users,
%and
%$6\%\sim30\%$ with $20\%$ video users.
%We can further find that the energy consumption reduction increases with the average link capacity, as a larger link capacity can achieve a more efficient cooperative scheduling.~~~~~~~ 
%}


\emph{3) \textbf{Algorithm Comparison:}}
From Figure \ref{fig:multiple-bitrate} (a) to (c) and
Figure \ref{fig:multiple-sw} (a) to (c), we can also evaluate the performance difference between our proposed algorithm and the   algorithms in \cite{b1} and \cite{b6} in the multi-user scenario.
Notice that the solid bars in Figure \ref{fig:multiple-bitrate} and
Figure \ref{fig:multiple-sw} are equivalent to the corresponding bars in Figure \ref{fig:single-real}, as the performance under the non-cooperative scenario in the multi-user scenario is equivalent to the performance in the single-user scenario.
By comparing the difference between solid bars (for the single-user scenario) and the difference between hollow bars (for the multi-user cooperative scenario), we can find that the performance difference (between our algorithm and the algorithms in \cite{b1, b6}) become more significant in the multi-user scenario, especially when the video user percentage is small.
For example, with $20\%$ video users, the average bitrate increase of our algorithm reaches $20\%\sim30\%$, and the average social welfare increase of our algorithm reaches
$10\%\sim50\%$.
Such an increasing in the performance difference (between our   algorithm and those in \cite{b1,b6}) is mainly due to the non-optimal segment owner selection in \cite{b1, b6}. In our algorithm, however, the segment owner selection and the bitrate adaptation are optimised jointly.

%\begin{table}[t]
%\vspace{-5mm}
%\centering
%\caption{Ratio of Energy Consumption under Cooperation and Non-Cooperation}
%\label{energy:tbl}
%\small
%\begin{tabular}{|c|c|c|c|}
%  \hline
%  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%User Scenarios &  Low Capacity (0-0.7Mbps) &   Middle Capacity (0-2.5Mbps) &   High Capacity (0-8.0Mbps)
%\\
%  \hline
%(a) 100\% Video Users & 99.2\% & 96.9\% & 87.4\%
%\\
%  \hline
%(b) 60\% Video Users & 95.7\% & 85.4\% &  78.3\%
%\\
%  \hline
%(c) 20\% Video Users & 93.9\% & 76.3\% &  70.2\%
%\\
%  \hline
%\end{tabular}
%\end{table}


%\emph{1) \textbf{Two Users under Full Encounter:}}
%Now we perform experiments for the multi-user scenario, where some users play  the high-resolution videos (bitrate $2.3$Mbps) while others remain idle and can potential help the encountered video users. The video configurations (such as video length, segment length, and buffer size) is same as those in the single-user case.
%We use these experiment to illustrate both the cooperation gain of our proposed crowdsourced system and the performance gain of our proposed algorithm.
%
%We first construct experiments for the single-user scenario (i.e., non-cooperative scenario), where the user plays a high-resolution video (bitrate $2.3$Mbps). The total video length is 500 seconds,  the segment length is 2 seconds, and the maximum  buffer length at the user's device is 40 seconds.
% {We use these experiments to illustrate the performance gap of our proposed Lyapunov-based online algorithm to the theoretical performance bound.
%We also use these experiments to compare the bitrate adaptation performance of our proposed algorithm with the existing online algorithms.}
%
%
%
%
%We then compare the performances of the online algorithms in the two-user case under full encounter.
%Namely, two users are encountered all the time, hence can cooperate with each other all the time.
%Both users play   high-resolution videos (bitrate $2.3$Mbps), with a total video length of 500 seconds,  a segment length of 5 seconds, and a maximum buffer length at the user's device of 100 seconds.
%
%Figure \ref{fig:multiple-real} shows the average (aggregate) bitrate and social welfare under realistic link capacities (extracted from real data traces).\scfootnote{To reduce the simulation complexity, we do not provide the offline theoretical performance upperbound. Actually, our proposed online algorithm can be viewed as an approximation to this bound, as their gap is very small (lower than $3\%$).}
%Note that the total average link capacity is the sum of both users' capacities.
%We can see from (a) that our proposed  algorithm (Blue) achieves
%an average bitrate much higher than other two  algorithm (with an average bitrate increase of $30\% \sim 50\%$).
%We can further see from (c) that our proposed algorithm achieves a social welfare higher than other two algorithms (with an average gain of  $10\% \sim 30\%$).
%
%
%
%\emph{2) \textbf{Multi-User under Real Mobility Traces:}}
%We now compare the performances of the online algorithms in the real multi-user scenario, i.e., under real mobility traces and measured throughput traces.
%Users move according to real mobility traces, and their link capacities are extracted from their measured throughput traces.
%Each user plays a 500 seconds video, and chooses  a quality (bitrate) randomly.
%
%
%
%Figure \ref{fig:many-real} shows the social welfare in such a real multi-user scenario under different number of users.
%Each point in subfigure (a) shows the total social welfare   generated  in one simulation round (corresponding to a particular selections of mobility traces, throughput traces, and video bitrates for all users) in a 5-user scenario.
%Subfigures (b) shows the average total social welfare in 1000 simulation rounds with the same number of users.
%We can see  that our proposed  algorithm (Blue) achieves  a social welfare  higher than   other two algorithms (with an average gain of $2\% \sim 15\%$).
%Moreover, the performance gain become more significant with a larger number of users.
%This implies that our proposed Lyapunov-based algorithm can better extract the cooperation gain in this crowdsourced system,  by the joint optimization of user selection and bitrate selection in each decision-making time.
%

